Parallel-R1: Towards Parallel Thinking via Reinforcement Learning

Parallel thinking has emerged as a novel approach for enhancing the reasoning capabilities of large language models (LLMs) by exploring multiple reasoning paths concurrently. However, activating such capabilities through training remains challenging, as existing methods predominantly rely on supervised fine-tuning (SFT) over synthetic data, which encourages teacher-forced imitation rather than exploration and generalization. Different from them, we propose \textbf{Parallel-R1}, the first reinforcement learning (RL) framework that enables parallel thinking behaviors for complex real-world reasoning tasks. Our framework employs a progressive curriculum that explicitly addresses the cold-start problem in training parallel thinking with RL. We first use SFT on prompt-generated trajectories from easier tasks to instill the parallel thinking ability, then transition to RL to explore and generalize this skill on harder problems. Experiments on various math benchmarks, including MATH, AMC23, and AIME, show that Parallel-R1 successfully instills parallel thinking, leading to 8.4% accuracy improvements over the sequential thinking model trained directly on challenging tasks with RL. Further analysis reveals a clear shift in the model's thinking behavior: at an early stage, it uses parallel thinking as an exploration strategy, while in a later stage, it uses the same capability for multi-perspective verification. Most significantly, we validate parallel thinking as a \textbf{mid-training exploration scaffold}, where this temporary exploratory phase unlocks a higher performance ceiling after RL, yielding a 42.9% improvement over the baseline on AIME25. Our model, data, and code will be open-source at https://github.com/zhengkid/Parallel-R1.

==> obs.tex <==
\section{Method}
\subsection{Overview}
%定义下问题，什么是GUI agent，The completion of a GUI task can be formulated as a Markov Decision Process(MDP)，根据这个出发，补充细节GUI action的细节，然后定义下notations，具体用什么notation跟我们最后一节GPRO training统一就好

%另起一段讲整个method的安排是啥
\subsection{Interactable Environment for Online Learning}
%传统方案主要是在pre-collected trajectory数据上训练所以模型可以探索的范围就被限制了，而且遇到现实环境中的弹窗之类的东西的话属于原始数据的out-of-distribution数据，也会处理起来有问题，所以我们的方案更好
Our framework is centered around an \textit{interactable environment} designed to support online reinforcement learning for mobile GUI agents. This environment facilitates continuous learning by allowing the agent to collect interaction data in real-time from high-fidelity, emulated mobile device interfaces.

The environment is architected as a scalable, batched system that manages numerous Android emulator instances in parallel, enabling high-throughput trajectory collection. To ensure authentic interactions, the system leverages a combination of low-level device controls and high-level automation frameworks, granting the agent comprehensive control over the GUI and underlying system functions. 
%This architecture is highly configurable, allowing for adjustments to the number of concurrent instances, maximum steps per episode, and screen resolution to suit various experimental requirements.

The agent interacts with the environment through a closed perception-action loop. At each timestep, the agent receives a multimodal observation comprising three key components: 1. \textbf{Visual Input}: the current device screenshot (visual state), 2. \textbf{Task Goal}: the natural language task instruction (goal), 3. \textbf{Interaction History}: a record of the agent's previous actions (context).

This information is processed by our vision-language model (VLM) agent, which first generates an internal reasoning trace before producing a structured action command. The agent’s action space is designed to cover a comprehensive range of mobile interactions and is categorized as follows: 1. \textbf{Physical Gestures}: parameterized actions such as taps and swipes, defined using normalized screen coordinates to ensure resolution independence. 2. \textbf{Text Input}: actions for entering text into active input fields. 3. \textbf{System Navigation}: device-level operations such as \texttt{Back}, \texttt{Home}, and \texttt{Enter}. 4. \textbf{Control and Temporal Actions}: meta-actions including \texttt{wait}, which enables synchronization with dynamic UI elements, and \texttt{terminate}, which ends the episode.

A sequence of these interactions forms a \textit{trajectory}, which is evaluated upon termination. Our framework employs an outcome-based reward mechanism, where the success of an entire trajectory is judged by an automated evaluation oracle. This oracle, which can be powered by a state-of-the-art vision-language model such as Qwen 2.5 VL 72B, analyzes the final $k$ screenshots of the trajectory in the context of the initial task instruction. By examining multiple final frames, the evaluator can verify completion of tasks that involve multi-step state changes.
The oracle returns a sparse, binary reward signal (1 for success, 0 for failure). This trajectory-level reward is then used to compute advantages for policy optimization.

\subsection{Synthetic Tasks for Mobile Agent Training}
\subsubsection{self-exploration for initial diverse data generation}
%根据以下的流程写个简略版本
%Step.1 An agent random walk in the environment.
%Step.2 A GPT4o will summarize the trajectories into tasks.
%Step.3.Reasonable tasks will be saved as our training data.
\subsubsection{Task Filtering via a Text-based World Model}
%把之前的定义的notation也安排进这一节里面
While self-exploration produces a diverse range of tasks, the raw outputs often contain considerable noise. Many synthesized tasks are either semantically ambiguous, as interpreted by the summarizing LLM, or inherently too complex for a moderately-sized MLLM agent (e.g., a 7B parameter model) to solve. Training on such tasks is inefficient—insurmountable tasks provide negligible learning signals, wasting computational resources and potentially destabilizing the training process. Therefore, a mechanism to filter raw tasks and curate a high-quality, difficulty-appropriate dataset is essential for effective online reinforcement learning.

To address this, we introduce a lightweight, simulation-based pre-assessment filter designed to estimate task solvability without incurring the high computational cost of executing full-scale GUI environment rollouts. At the core of this filter is a powerful LLM, specifically GPT-4o, which acts as a \textit{text-based world model}. This model simulates the Android GUI environment by generating structured, textual descriptions of screen states in response to agent actions.

The filtering procedure is implemented as a zero-shot, text-only interaction loop between a simulated agent and the world model, consisting of the following steps:

\begin{enumerate}
    \item \textbf{Initialization:} The world model is provided with a candidate task (e.g., \textit{``Set a timer for 5 minutes''}) and generates a textual description of the initial screen state. This description is formatted as a list of UI elements, each with associated content descriptions, types, and estimated coordinates.
    
    \item \textbf{Agent Action:} A proxy agent, configured to emulate the reasoning capabilities of the target MLLM, receives the screen description. It formulates a plan and outputs an action in a structured format (e.g., \texttt{\{"action": "click", "coordinates": [x, y]\}}).
    
    \item \textbf{State Transition:} The world model receives the agent's action, simulates its outcome, and generates a new textual description of the resulting screen state. For example, after clicking the ``Clock'' icon, the model may describe the interface of the Clock application.
    
    \item \textbf{Feasibility Assessment:} This interaction continues iteratively until the agent outputs a \texttt{terminate(success)} action, signals failure, or exceeds a predefined step limit.
\end{enumerate}

A task is admitted into the training set only if the simulation concludes in \textit{success} state within the step limit. This process effectively filters out tasks that are logically convoluted or overly long, serving as a proxy for complexity. By decoupling reasoning and planning from visual perception, this simulation-based filtering provides a strong, low-cost signal for identifying tasks within the agent’s current capability range. As a result, the online learning phase is focused on a curriculum of achievable yet challenging tasks, maximizing the efficiency and effectiveness of our MoGUI-RL framework.

\subsection{Online Learning with GRPO}
% Should we come with another *PO name for this part?
%design to adapt the GPRO to GUI agent training, each
% issue with naive adaptation? 1. advantage disappearing issue(as long as one trajectory win, the reward is 1, but for short trajectories, the better) 2. Self-termination leads to early stopping: (the temination is issued by the agent, sometimes it calls temination too early) 3. Thinking too short.
To optimize the policy of a GUI-based agent over multi-step trajectories, we adapt the Generalized Reward-Policy Optimization (GRPO) objective to incorporate trajectory structure and outcome-driven credit assignment. The proposed GUI-GRPO loss is defined as:
\begin{equation*}
\mathcal{L}_{\text{GUI-GRPO}} = -\frac{1}{\sum_{t=1}^{G}|\mathbf{o}_{i,s}|} \sum_{i=1}^{G} \sum_{s=1}^{S_i}  \sum_{t=1}^{|\mathbf{o}_{i,s}|} 
\left\{
\min \left[
\frac{\pi_{\theta}(o_{i,s,t} \mid \mathbf{q}, \mathbf{h}_{i,s}, \mathbf{o}_{i,s,<t})}{\pi_{\theta_{\text{old}}}(o_{i,s,t} \mid \mathbf{q}, \mathbf{h}_{i,s}, \mathbf{o}_{i,s,<t})} \hat{A}_{i,s,t}, \,
\text{clip}\left(
\frac{\pi_{\theta}(o_{i,s,t} \mid \mathbf{q}, \mathbf{h}_{i,s}, \mathbf{o}_{i,s,<t})}{\pi_{\theta_{\text{old}}}(o_{i,s,t} \mid \mathbf{q}, \mathbf{h}_{i,s}, \mathbf{o}_{i,s,<t})},
1 - \epsilon, 1 + \epsilon
\right) \hat{A}_{i,s,t}
\right]
\right\}
\end{equation*}
where $G$ is the number of sampled trajectories per task prompt $\mathbf{q}$, $S_i$ denotes the number of steps in trajectory $i$, and $\mathbf{o}{i,s}$ is the model-generated response at step $s$ of trajectory $i$, tokenized as ${o{i,s,1}, \ldots, o_{i,s,T}}$. Each token-level log probability is weighted by a shared advantage $\hat{A}_{i,s,t}$ computed at the trajectory level.

We define the normalized advantage as:

\begin{equation*}
\hat{A}{i,s,t} = \frac{R_i^{\text{max}} - \mu{\mathbf{q}}}{\sigma_{\mathbf{q}} + \epsilon},
\end{equation*}

where $R_i^{\text{max}} = \max_{s=1}^{S_i} R(\mathbf{q}, \text{traj}i, s)$ denotes the maximum reward obtained across all steps of trajectory $i$, $\mu{\mathbf{q}} = \frac{1}{G} \sum_{j=1}^{G} R_j^{\text{max}}$ is the mean of maximum rewards across all sampled trajectories for prompt $\mathbf{q}$, and $\sigma_{\mathbf{q}}$ is their standard deviation.

This formulation introduces several key modifications over standard GRPO:

Trajectory-level Advantage Estimation: Rewards are assigned based on the best-performing step in each trajectory, providing a stable and outcome-aware credit signal.

Step-wise Action Evaluation: The loss aggregates over multiple steps, enabling the agent to learn from long-horizon interactions.

Token-level Optimization: Each action (token) within a step is updated using the same trajectory-level advantage, encouraging consistency across the entire decision sequence.

Together, these adaptations make GUI-GRPO particularly suitable for reinforcement learning tasks in GUI environments where rewards are sparse and trajectory quality varies significantly across interaction steps.


We propose a novel reward formulation for training GUI agents that extends the standard GRPO framework to incorporate cognitive reasoning processes and efficiency constraints. Our approach addresses the unique challenges of GUI navigation, where both task completion accuracy and trajectory efficiency are critical for practical deployment.

\subsubsection{Multi-Component Reward Formulation}

Let $\mathcal{T}$ denote a GUI task, and $\tau = (s_0, a_0, s_1, a_1, ..., s_T, a_T)$ represent a trajectory of states and actions. We design a composite reward function $r(\tau, \mathcal{T})$ that consists of four key components:

\begin{equation}
r(\tau, \mathcal{T}) = \begin{cases}
r_{\text{base}} \cdot \alpha_{\text{steps}} + r_{\text{think}} & \text{if task completed successfully} \\
-\beta_{\text{premature}} & \text{if premature termination} \\
0 & \text{otherwise}
\end{cases}
\end{equation}

where $r_{\text{base}} \in \{0, 1\}$ indicates task success, $\alpha_{\text{steps}}$ is an efficiency scaling factor, $r_{\text{think}}$ rewards reasoning quality, and $\beta_{\text{premature}}$ penalizes incorrect termination.

\subsubsection{Efficiency-Aware Step Scaling}

A key innovation in our approach is the introduction of an exponential decay factor that encourages agents to complete tasks with minimal steps. This design is motivated by the observation that shorter trajectories typically contain fewer compounding errors and provide better user experience. We define the efficiency scaling factor as:

\begin{equation}
\alpha_{\text{steps}} = \text{clip}\left(e^{-\lambda \cdot |\tau|}, \alpha_{\min}, \alpha_{\max}\right)
\end{equation}

where $|\tau|$ denotes the trajectory length, $\lambda > 0$ is the decay factor controlling the penalty strength, and $[\alpha_{\min}, \alpha_{\max}]$ bounds the scaling factor. This exponential formulation ensures that:
\begin{itemize}
    \item Early task completion receives substantially higher rewards
    \item The penalty increases smoothly with trajectory length
    \item Extreme penalties are avoided through clipping
\end{itemize}

\subsubsection{Cognitive Process Modeling}

Unlike traditional RL approaches that focus solely on action outcomes, we explicitly model and reward the agent's reasoning process. Let $\mathcal{C}_t$ denote the thinking content generated at step $t$. We compute the thinking reward as:

\begin{equation}
r_{\text{think}} = \gamma \cdot \sigma\left(\frac{\bar{n}_{\text{tokens}} - \mu_{\max}/2}{\mu_{\max}/4}\right)
\end{equation}

where $\bar{n}_{\text{tokens}} = \frac{1}{|\tau|}\sum_{t=0}^{|\tau|} |\mathcal{C}_t|$ represents the average thinking tokens per step, $\mu_{\max}$ is the expected maximum tokens, $\gamma$ is a scaling factor, and $\sigma(\cdot)$ is the sigmoid function. This formulation encourages consistent reasoning throughout the trajectory while maintaining bounded rewards.

\subsubsection{Premature Termination Penalty}

To discourage hasty task termination and promote thorough exploration, we introduce a penalty that decreases with trajectory length:

\begin{equation}
\beta_{\text{premature}} = \beta_{\max} \cdot \left(1 - \frac{|\tau|}{T_{\max}}\right)
\end{equation}

where $\beta_{\max}$ is the maximum penalty and $T_{\max}$ is the maximum allowed steps. This formulation acknowledges that termination attempts after more exploration are more likely to be justified.

\subsubsection{Integration with GRPO}

The advantage computation in our modified GRPO framework incorporates trajectory-level optimization. For a batch of trajectories $\{\tau_i\}_{i=1}^G$ generated for task $\mathcal{T}$, we compute advantages as:

\begin{equation}
\hat{A}_{i,s,t} = \frac{r^{\max}_i - \mu_{\mathcal{T}}}{\sigma_{\mathcal{T}} + \epsilon}
\end{equation}

where $r^{\max}_i = \max_{s \in \tau_i} r(s, \mathcal{T})$ represents the maximum reward achieved in trajectory $i$, and $\mu_{\mathcal{T}}$, $\sigma_{\mathcal{T}}$ are the mean and standard deviation of maximum rewards across all trajectories for task $\mathcal{T}$.

This formulation enables the agent to learn from both successful task completions and the efficiency of execution paths, leading to more robust and practical GUI navigation policies. The exponential decay in step scaling particularly encourages the discovery of direct navigation paths, which is crucial for real-world deployment where user experience depends heavily on task completion speed.


While self-exploration can produce a diverse set of task instructions, we found that many of them are either too ambiguous due to the LLM’s summarization limitations or too complex to complete, given the current state of the GUI. Asking the agent to generate trajectories on such impossible tasks wastes computational resources, and these trajectories can destabilize the learning process. We introduce a novel filtering mechanism using a text-based world model that efficiently pre-screens tasks without expensive environment rollouts.


% \begin{equation}
% \mathcal{L}_{\text{GUI-GRPO}} = -\mathbb{E}_{\tau \sim \pi_{\theta_{\text{old}}}} \left[ \sum_{s=1}^{|\tau|} \sum_{t=1}^{|a_s|} \min \left( r_t(\theta) \hat{A}_{\tau}, \text{clip}(r_t(\theta), 1-\epsilon, 1+\epsilon) \hat{A}_{\tau} \right) \right]
% \end{equation}


%The reasoning reward $r_{\text{reasoning}}(\tau) = \gamma \cdot \sigma\left(\frac{\bar{n}_{\text{tokens}} - \mu_{\max}/2}{\mu_{\max}/4}\right)$ encourages the agent to maintain thoughtful reasoning throughout the trajectory. Here, $\bar{n}_{\text{tokens}}$ represents the average reasoning length per step, and the sigmoid function ensures bounded contributions. This component is crucial for developing interpretable agents that can explain their actions.


The key innovation is our trajectory-level advantage computation that provides a consistent learning signal across all actions in a trajectory:

\begin{equation}
\hat{A}_{\tau} = \frac{R_{\tau}^{\max} - \bar{R}_{\mathbf{q}}}{\sigma_{R_{\mathbf{q}}} + \epsilon}
\end{equation}

where $R_{\tau}^{\max} = \max_{s \in \tau} R(s, \mathbf{q})$ captures the best outcome achieved in the trajectory, $\bar{R}_{\mathbf{q}}$ and $\sigma_{R_{\mathbf{q}}}$ are the mean and standard deviation of maximum rewards across all trajectories for task $\mathbf{q}$. This formulation ensures that successful trajectories receive positive advantages regardless of when success occurs, addressing the credit assignment problem in long-horizon tasks.


\subsubsection{Multi-Component Reward Design}
GUI navigation requires balancing multiple objectives: completing the task correctly, doing so efficiently, and maintaining interpretable reasoning. We design a composite reward function that captures these dimensions:

\begin{equation}
R(\tau, \mathbf{q}) = \begin{cases}
r_{\text{base}} \cdot f_{\text{efficiency}}(|\tau|) & \text{if success} \\
-\beta \cdot g(|\tau|) & \text{if premature termination} \\
0 & \text{otherwise}
\end{cases}
\end{equation}

The efficiency factor $f_{\text{efficiency}}(|\tau|) = \text{clip}(e^{-\lambda|\tau|}, \alpha_{\min}, \alpha_{\max})$ implements an exponential decay that strongly incentivizes shorter trajectories. This design reflects the reality that efficient GUI navigation improves user experience and reduces compounding errors. The decay rate $\lambda$ controls the strength of this preference, while clipping prevents extreme penalties that could discourage exploration.

The premature termination penalty $\beta \cdot g(|\tau|) = \beta_{\max}(1 - |\tau|/T_{\max})$ discourages hasty task abandonment while acknowledging that later termination attempts are more likely justified. This graduated penalty prevents the agent from developing a bias toward early termination when facing challenging tasks.

Together, these components create a rich learning signal that guides the agent toward efficient, successful, and interpretable GUI navigation strategies. The multi-component design allows fine-tuning the balance between different objectives through hyperparameters, enabling adaptation to specific deployment requirements.

% \begin{table*}[htp]
% \centering
% \caption{Performance on GUI Agent benchmarks. TM = Type Match, EM = Exact Match, SR = Success Rate.} %Bold and \underline{underline} indicate best and second-best results.}
% \begin{tabular}{lcccccccc}
% \toprule
% \textbf{Models} & \textbf{AW} & \multicolumn{2}{c}{\textbf{AC-High}} & \multicolumn{2}{c}{\textbf{AITZ}} & \textbf{AITW-Gen} & \textbf{AITW-Web} \\
%  & SR & TM & EM & TM & EM & SR & SR \\
% \midrule
% \multicolumn{8}{l}{\textit{Closed-source Models}} \\
% GPT-4o~\citep{hurst2024gpt} & 34.5 & 20.8 & - & 70.0 & 35.3 & - & - \\
% Gemini 2.0~\citep{deepmind2024gemini} & - & 60.2 & - & - & - & - & - \\
% Claude 3.5~\citep{anthropic2024claude35} & - & 12.5 & - & - & - & - & - \\
% \midrule
% \multicolumn{8}{l}{\textit{Open-source 7B Models}} \\
% Qwen2.5-VL-7B~\citep{bai2025qwen2} & 22.0 &75.1   &62.9   &78.4   &54.6   &  &  \\
% OS-Genesis-7B~\citep{sun2024genesis} & - &65.9   &44.4   &20.0   &8.45   & - & - \\
% OS-Atlas-7B~\citep{wu2024atlas} & -  &70.4   &56.5   &74.1   &58.5  & - & -\\
% Aguvis-7B~\citep{huang2024understanding} & - &58.8  & 32.7  &59.2   &31.6   & - & - \\
% UI-TARS-7B~\citep{qin2025ui} & 33.0 &81.6 &74.4  &80.4  &65.8   &  & \\
% \textbf{MoGUI 7B (Ours)} & 30.0 &75.9  &63.0  &77.8  &62.9 &  & \\
% \midrule
% \multicolumn{8}{l}{\textit{Open-source 32B/72B Models}} \\
% Qwen2.5-VL-32B~\citep{bai2025qwen2} &31.5
%   &   &   &   &   & - & - \\
% Qwen2.5-VL-72B~\citep{bai2025qwen2} &  &   &   &   &   & - & - \\
% UI-TARS-72B~\citep{qin2025ui} & 46.6 &   &  &   &   & - & - \\
% Aguvis-72B~\citep{huang2024understanding} & 26.1 &   &   &  &   &  & \\
% \textbf{MoGUI 32B (Ours)} & 44.8 &79.7  &67.2  &77.7  &63.0 &  &  \\
% \bottomrule
% \end{tabular}
% \label{tab:mogui-expanded}
% \end{table*}

% \begin{table*}[htp]
% \centering
% \caption{Performance on GUI Agent benchmarks. TM = Type Match, EM = Exact Match, SR = Success Rate.}
% \begin{tabular}{lcccccc}
% \toprule
% \textbf{Models} & \textbf{AW} & \multicolumn{2}{c}{\textbf{AC-High}} & \multicolumn{2}{c}{\textbf{AITZ}} \\
%  & SR & TM & EM & TM & EM \\
% \midrule
% \multicolumn{7}{l}{\textit{Closed-source Models}} \\
% GPT-4o~\citep{hurst2024gpt} & 34.5 &-  &  20.8& 70.0 & 35.3 \\
% Gemini 2.0~\citep{deepmind2024gemini} & - & - & 60.2 & - & - \\
% Claude 3.5~\citep{anthropic2024claude35} & - & - & 12.5 & - & - \\
% \midrule
% \multicolumn{7}{l}{\textit{Open-source Models}} \\
% Qwen2.5-VL-7B~\citep{bai2025qwen2} & 22.0 & 69.7 & 57.4 & 73.2 & 57.6 \\
% OS-Genesis-7B~\citep{sun2024genesis} & - & 65.9 & 44.4 & 20.0 & 8.45 \\
% OS-Atlas-7B~\citep{wu2024atlas} & - & 70.4 & 56.5 & 74.1 & 58.5 \\
% Aguvis-7B~\citep{huang2024understanding} & - & 58.8 & 32.7 & 59.2 & 31.6 \\
% %UI-TARS-7B~\citep{qin2025ui} & 33.0 & 81.6 & 74.4 & 80.4 & 65.8 \\
% Qwen2.5-VL-32B~\citep{bai2025qwen2} & 31.5 &78.8  &74.1  &78.8  &64.5  \\
% \textbf{MobileGUI-7B (Ours)} & 30.0 & 75.9 & 63.0 & 77.8 & 62.9 \\
% \textbf{MobileGUI-32B (Ours)} & 44.8 & 79.7 & 67.2 & 77.7 & 63.0 \\
% \bottomrule
% \end{tabular}
% \label{tab:mogui-expanded}
% \end{table*}

% On the challenging AndroidWorld (AW) benchmark, our MobileGUI-32B agent achieves a new state-of-the-art Success Rate (SR) of 44.8\%. This marks a substantial improvement of 13.3 absolute points over its base model, Qwen2.5-VL-32B (31.5\% SR), and significantly outperforms the strongest closed-source model, GPT-4o (34.5\% SR). Similarly, MobileGUI-7B improves its base model's SR from 22.0\% to 30.0\%, demonstrating the effectiveness of MobileGUI-RL on different model scales.

% On the AndroidControl-High (AC-High) and Android-in-the-Zoo (AITZ) benchmarks, our models show consistent improvements in reasoning and precise interaction. For instance, MobileGUI-7B improves the Exact Match (EM) score on AITZ from 54.6\% to 62.9\% compared to its base model. Also, our MobileGUI agents consistently elevate the performance of the underlying Qwen2.5-VL models. 
% Overall, the results validate that training with MobileGUI-RL leads to more capable and robust GUI agents. The framework effectively enhances the models' ability to complete complex tasks, with the most significant gains observed in the largest model, highlighting the synergy between model scale and our online reinforcement learning approach.
